EVEDIT: Event-based Knowledge Editing with Deductive Editing Boundaries

The dynamic nature of real-world information necessitates efficient knowledge editing (KE) in large language models (LLMs) for knowledge updating. However, current KE approaches, which typically operate on (subject, relation, object) triples, ignore the contextual information and the relation among different knowledge. Such editing methods could thus encounter an uncertain editing boundary, leaving a lot of relevant knowledge in ambiguity: Queries that could be answered pre-edit cannot be reliably answered afterward. In this work, we analyze this issue by introducing a theoretical framework for KE that highlights an overlooked set of knowledge that remains unchanged and aids in knowledge deduction during editing, which we name as the deduction anchor. We further address this issue by proposing a novel task of event-based knowledge editing that pairs facts with event descriptions. This task manifests not only a closer simulation of real-world editing scenarios but also a more logically sound setting, implicitly defining the deduction anchor to address the issue of indeterminate editing boundaries. We empirically demonstrate the superiority of event-based editing over the existing setting on resolving uncertainty in edited models, and curate a new benchmark dataset EvEdit derived from the CounterFact dataset. Moreover, while we observe that the event-based setting is significantly challenging for existing approaches, we propose a novel approach Self-Edit that showcases stronger performance, achieving 55.6% consistency improvement while maintaining the naturalness of generation.

==> Contents/Formulation_new.tex <==
\section{Fallacies of Knowledge Editing}
\label{formulation}
In this section, we formulate and analyze the task of knowledge editing from a theoretical perspective. In \S~\ref{sec:knowledge}, we present a formulation for knowledge and knowledge boundaries. In \S~\ref{sec:deficiency}, we theoretically analyze the fallacies of current knowledge editing settings.

\subsection{Formulation of Knowledge Editing}
\label{sec:knowledge}
We present a theoretical framework for knowledge editing based on the \emph{formal logic}~\cite{smith2003introduction} where we consider \emph{knowledge} as \emph{propositions}\footnote{Propositions are arguments that can be either true or false}. For a knowledge system, the purpose of knowledge editing is to alter its set of knowledge. Therefore, we first formally define the knowledge within a system and the knowledge edit.

\begin{definition}[Knowledge of Systems]
    The \emph{knowledge} of a system is a set of propositions that is considered true in the system.
\end{definition}

To align the theoretical framework with the editing of language models, we introduce the knowledge of language models. Let $k$ denote a proposition, and let $\Theta$ represent a language model. We assess whether $\Theta$ "possesses" knowledge of $k$ by calculating $P(y_k|x_k, \Theta)$, where $(x_k, y_k)$ represents a pair of input-output tokens designed for verification purposes. We opt for $P(y_k|x_k, \Theta)$ over $P(k|\Theta)$ because the probability assigned by a language model to a proposition does not inherently correlate with its logical validity~\cite{yu2023self}
\begin{definition}[Knowledge of LMs]
For a language model $\Theta$, the universe of all conceivable knowledge $\mathcal{U}$, and a threshold $\varepsilon$ within the range $[0, 0.5)$, the set of knowledge recognized by $\Theta$ is
\begin{equation}
\mathcal{K}_{\Theta,\varepsilon} = \{k\in\mathcal{U}|P(y_k|x_k, \Theta) \ge 1 - \epsilon\}.
\end{equation}
\end{definition}

In this work, we are specifically concerned with the logical deduction during editing. An example of logical deduction is
\begin{quote}
\begin{centering}
    $P:$ The city Tom was born is New York\\
    $Q:$ The country of New York is U.S.\\
    $\downarrow$\\
    $X:$ The country Tom was born is U.S.\\
\end{centering}
\end{quote}
For a knowledge set $\mathcal{K}$, its \emph{deductive closure} $\mathcal{B}(\mathcal{K})$ is the set of all propositions logically entailed  by $\mathcal{K}$. $\mathcal{K}$ is \emph{deductively closed}, or simply \emph{closed}, if and only if $\mathcal{B}(\mathcal{K}) = \mathcal{K}$. Determining the deductive closure presents a significant challenge due to the difficulty in formulating inference rules~\cite{smith2003introduction}. However, given the advanced in-context reasoning capabilities demonstrated by large language models, we establish the deductive closure based on such in-context deduction.
\begin{definition}[In-context Deductive Closure]
For any given set of knowledge $\mathcal{K}$, its In-context Deductive Closure as provided by a language model $\Phi$ is the set of knowledge that can be deduced,
\begin{equation}\label{eq:def_ictdc}
\mathcal{B}_{\Phi,\epsilon}(\mathcal{K})=\{u\in\mathcal{U}|P(y_u|x_u, \mathcal{K}, \Phi) \ge 1 - \epsilon\}. 
\end{equation}
\end{definition}
We assume a language model being edited to contain closed set of knowledge. Let $\mathcal{K}$ be the knowledge set of the pre-edit model, and $\mathcal{E}$ be the set of editing knowledge. We define two novel concepts for the soundness of editing: \emph{deduction closure} and \emph{editing boundary}.
\begin{definition}[Deduction Anchor of Editing] The \emph{deduction anchor} of an edit is a subset of the current knowledge assumed true throughout editing.
\end{definition}
We denote the deduction anchor by $\mathcal{K}^\mathcal{E}$, which serves as the base for generalization of the editing knowledge. We further define the editing boundary.
\begin{definition}[Editing Boundary]
    The editing boundary is the closed set $\mathcal{B}\left(\mathcal{K}^\mathcal{E}\cup \mathcal{E}\right)$ of logically relevant knowledge to the edit $\mathcal{E}$.
\end{definition}
% \begin{itemize}
    % \item \emph{Deduction Anchor} $\mathcal{K}^\mathcal{E}\subset \mathcal{K}$ is an ``static'' subset of the current knowledge set that remains true in the post-editing model. While the choice of $\mathcal{K}^\mathcal{E}$ can be arbitrary, we will show that a proper assignment is indispensable for knowledge generalization in \S~\ref{sec:deficiency}.
    % \item \emph{Editing Boundary} .
% \end{itemize}
We thereby define \emph{knowledge editing}.
\begin{definition}[Knowledge Editing] Given the knowledge set $\mathcal{K}$, the edit $\mathcal{E}$ and the deduction anchor $\mathcal{K}^\mathcal{E}$, \emph{knowledge editing} is the process of computing post-edit knowledge set $\mathcal{K}'$:
    \begin{equation}\label{eq:def_ke}
    \begin{aligned}
        \mathcal{K}^D &= \left\{p\in\mathcal{K}| \neg p\in  \mathcal{B}\left(\mathcal{K}^\mathcal{E}\cup \mathcal{E}\right) \right\}\\
        \mathcal{K}' &= \mathcal{B}\left(\mathcal{K}\backslash\mathcal{K}^D \cup \mathcal{E}\right)
    \end{aligned},
\end{equation}
where $\mathcal{K}^\mathcal{E}$ satisfies that
\begin{equation}\label{eq:req_da}
    \forall k \in \mathcal{B}\left(\mathcal{K}\backslash\mathcal{K}^D\right), \neg k \notin \mathcal{B}\left(\mathcal{K}^\mathcal{E}\cup \mathcal{E}\right) .
\end{equation}
Here Equation~(\ref{eq:req_da}) ensures the consistency of $\mathcal{K}'$.
\end{definition}
% Utilizing the defined concepts of knowledge and deductive closure, 
We also define knowledge editing of language models. It's important to note that the model used to determine deductive closure serves only in defining the task and not in the editing process itself. Thus, it may differ from the model undergoing edits. For instance, a more capable model may be employed for a  better deductive closure. % for evaluation purposes.
\begin{definition}[Knowledge Editing of LMs]
    Following the notations in Equation~(\ref{eq:def_ke}), to edit a language model $\Theta$ based on the in-context deductive closure provided by $\Phi$ involves identifying a modified model $\Theta'$ such that
    \begin{equation}
    \begin{aligned}
        \mathcal{K}^D &= \left\{p\in\mathcal{K}_{\Theta,\varepsilon_\Theta}| \neg p\in  \mathcal{B}_{\Phi, \varepsilon_\Phi}\left(\mathcal{K}^\mathcal{E}\cup \mathcal{E}\right) \right\}\\
        \mathcal{K}' &= \mathcal{B}_{\Phi, \varepsilon_\Phi}\left(\mathcal{K}_{\Theta,\varepsilon_\Theta}\backslash\mathcal{K}^D \cup \mathcal{E}\right)
    \end{aligned}.
    \end{equation}
\end{definition}
\begin{comment}
To align the theoretical framework with the editing of language models, we introduce specific terminology mappings.
\paragraph{Knowledge of LMs}  Let $k$ denote a proposition or a piece of knowledge, and let $\Theta$ represent a language model. We assess whether $\Theta$ "possesses" knowledge of $k$ by calculating $P(y_k|x_k, \Theta)$, where $(x_k, y_k)$ represents a pair of input-output tokens designed for verification purposes. We opt for $P(y_k|x_k, \Theta)$ over $P(k|\Theta)$ because the probability assigned by a language model to a proposition does not inherently correlate with its logical validity~\cite{yu2023self}.
\begin{definition}[Knowledge of LMs]
For a language model $\Theta$, the universe of all conceivable knowledge $\mathcal{U}$, and a threshold $\varepsilon$ within the range $[0, 0.5)$, the set of knowledge recognized by $\Theta$ is
\begin{equation}
\mathcal{K}_{\Theta,\varepsilon} = \{k\in\mathcal{U}|P(y_k|x_k, \Theta) \ge 1 - \epsilon\}.
\end{equation}
\end{definition}
\paragraph{Deductive Closure of LMs} Determining the deductive closure presents a significant challenge due to the difficulty in formulating inference rules~\cite{smith2003introduction}. However, given the advanced in-context reasoning capabilities demonstrated by large language models, we establish the deductive closure based on such in-context deduction.
\begin{definition}[In-context Deductive Closure]
For any given set of knowledge $\mathcal{K}$, its In-context Deductive Closure as provided by a language model $\Phi$ is the set of knowledge that can be deduced,
\begin{equation}\label{eq:def_ictdc}
\mathcal{B}_{\Phi,\epsilon}(\mathcal{K})=\{u\in\mathcal{U}|P(y_u|x_u, \mathcal{K}, \Phi) \ge 1 - \epsilon\}. 
\end{equation}
\end{definition}

\paragraph{Knowledge Editing of LMs} Utilizing the defined concepts of knowledge and deductive closure, we can outline the process of editing knowledge in language models. It's important to note that the model used to determine deductive closure serves only in defining the task and not in the editing process itself. Thus, it may differ from the model undergoing edits. For instance, a more capable model may be employed to achieve a  better deductive closure for evaluation purposes.
\begin{definition}[Knowledge Editing of LMs]
    Following the notations in Equation~(\ref{eq:def_ke}), to edit a language model $\Theta$ based on the in-context deductive closure provided by $\Phi$ involves identifying a modified model $\Theta'$ such that
    \begin{equation}
    \begin{aligned}
        \mathcal{K}^D &= \left\{p\in\mathcal{K}_{\Theta,\varepsilon_\Theta}| \neg p\in  \mathcal{B}_{\Phi, \varepsilon_\Phi}\left(\mathcal{K}^\mathcal{E}\cup \mathcal{E}\right) \right\}\\
        \mathcal{K}' &= \mathcal{B}_{\Phi, \varepsilon_\Phi}\left(\mathcal{K}_{\Theta,\varepsilon_\Theta}\backslash\mathcal{K}^D \cup \mathcal{E}\right)
    \end{aligned}.
    \end{equation}
\end{definition}
% We define the part of knowledge $\mathcal{K}$ that stayed unchanged during the edit process as $\mathcal{K}^R$ while the other part of knowledge that is updated as $\mathcal{K}^D$. The knowledge editing task is then defined as:
% We show that this concept of knowledge can be well mapped to the knowledge of language models. Based on this concept, we further define the deductive closure of knowledge sets.

% It is worth noticing that $\Phi$ can be different from the model being edited,  

% \paragraph{Mapping Propositions to LM Knowledge} This formulation encompasses previous triple-based formulation of the knowledge within language models by properly choosing $(x_k, y_k)$.\jiateng{is this sentence important ?}



% \subsection{Knowledge Editing}
% \label{sec:knowledge editing}
% \begin{equation}\label{eq:def_ke}
%     \begin{aligned}
%         \mathcal{K}^R &= \left\{p\in\mathcal{K}| \neg p\notin \mathcal{B}\left( \mathcal{E}\right) \right\}\\
%         \mathcal{K}^\mathcal{E} &= \mathcal{B}\left(\mathcal{K}^Rml;m \cup \mathcal{E}\right)
%     \end{aligned}.
% \end{equation}
% % , also following~\cite{cohen2023evaluating}
% \begin{equation}
%     \mathcal{K}^\mathcal{E} = \mathcal{B}\left(\mathcal{K}^R \cup \mathcal{E}\right)
% \end{equation}
% While some knowledge in $\mathcal{K}^R$  are useful in logical deductions, others is unrelated to the edit. We further define \textbf{static knowledge} $\mathcal{K}^S \in \mathcal{K}^R$, where
% \begin{equation}
%     \mathcal{B}\left(\mathcal{K}^S \cup \mathcal{E}\right) \cup \left(\mathcal{K}^R \setminus \mathcal{K}^S\right)  = \mathcal{B}\left(\mathcal{K}^R \cup \mathcal{E}\right)
% \end{equation}
\end{comment}
\subsection{Fallacies of Existing Knowledge Editing}
\label{sec:deficiency}

% From the above formulation, we identify two major logical fallacies in the existing setting. 
Existing work predominantly ignores the significance of the deduction anchor and resulting editing boundary. However, we present the following theorem, emphasizing the importance of choosing an appropriate set of $\mathcal{K^\mathcal{E}}$.
\begin{theorem}[Knowledge Explosion]
    If Equation~(\ref{eq:req_da}) is not satisfied, the post-editing knowledge set $\mathcal{K}'=\mathcal{U}$ where $\mathcal{U}$ is the universe of all knowledge, meaning any proposition is logically true.
\end{theorem}

% \begin{equation}
% \begin{aligned}
%     \exists k \in \mathcal{B}\left(\mathcal{K}\backslash\mathcal{K}^D\right)&\subset \mathcal{B}\left(\mathcal{K}\backslash\mathcal{K}^D \cup \mathcal{E}\right),\\
%     \neg k \in \mathcal{B}\left(\mathcal{K}^\mathcal{E}\cup \mathcal{E}\right)&\subset \mathcal{B}\left(\mathcal{K}\backslash\mathcal{K}^D \cup \mathcal{E}\right)
% \end{aligned}
% \end{equation}
% Due to \emph{ex falso quodlibet}, $\mathcal{K}'=\mathcal{B}\left(\mathcal{K}\backslash\mathcal{K}^D \cup \mathcal{E}\right)=\mathcal{U}$ where $\mathcal{U}$ is the universe of all knowledge, meaning any propositions should be logically true in the post-edit model. 
% \paragraph{No-Anchor Fallacy} 
While explicit definitions of deduction anchor or editing boundary is typically absent, existing work that merely focus on local edits assumes $\mathcal{K}^\mathcal{E} = \varnothing$, which limits the editing boundary $\mathcal{B}\left(\mathcal{K}^\mathcal{E} \cup \mathcal{E}\right)=\mathcal{B}\left(\mathcal{E}\right)$ to only contain paraphrases of $\mathcal{E}$, as the \emph{edit scope} proposed by \citet{mitchell2022memory}. Additionally, \citet{cohen2023evaluating} implicitly assumes that all the knowledge not directly conflicting with $\mathcal{E}$ as the deduction anchor. We have the following results for their fallacies.
\begin{theorem}[No-Anchor Fallacy] For an counterfactual and non-global edit $\mathcal{E}$, there exists at least one proper choice of $\mathcal{K}^\mathcal{E}\in2^\mathcal{K}$ satisfying Equation~(\ref{eq:req_da}), while $\varnothing$ does not.
\end{theorem}
\begin{theorem}[Maximum-Anchor Fallacy] For an counterfactual and non-local edit $\mathcal{E}$, there exists at least one proper choice of $\mathcal{K}^\mathcal{E}\in2^\mathcal{K}$ satisfying Equation~(\ref{eq:req_da}), while the following maximum anchor
\begin{equation}
    \mathcal{K}^\mathcal{E} = \{p\in\mathcal{K}| \neg p \notin \mathcal{B}(\mathcal{E})\}
\end{equation}
does not satisfy Equation~(\ref{eq:req_da}).
\end{theorem}
Here an \emph{counterfactual}, \emph{non-global} and \emph{non-local} edit is the one that contradicts with some but not all of the pre-editing knowledge. The rigorous definition is presented with proof in Appendix.
% We demonstrate that the empty deduction anchor does not satisfy Equation~(\ref{eq:req_da}) for counterfactual edits in Appendix. 

Moreover, the no-anchor fallacy leads to the shrinkage of knowledge set for the in-context deductive closure in Equation~(\ref{eq:def_ictdc}). The reason is that for two conflicting knowledge $p, q$ satisfying $x_p=x_q, y_p\ne y_q$, a language model cannot give $P(y_p|x_p) \ge 1 - \varepsilon$ and $P(y_q|x_q) \ge 1 - \varepsilon$ at the same time. Consequently, we hypothesize that both probabilities will go under the threshold of $1 - \varepsilon$, resulting in the loss of both knowledge and an increase of the answer entropy. We empirically verify this no-anchor fallacy for counterfactual edits. Specifically, we consider a set of paired edits and relevant queries of knowledge as follows:
\begin{quote}
    \textbf{Edit} $e$: \emph{City A} is located beside \emph{City B}.\\
    \textbf{Query} $q$: \emph{City A} is located in the country of \_\_\_
\end{quote}
where City A and City B are two cities in different countries. We show in Table that $P(\cdot|q)$ demonstrates a much stronger certainty compared with $P(\cdot|q, e)$

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\textwidth]{Inserts/uncertainty.pdf}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure*}


% as knowledge in $\mathcal{K}\\mathcal{K}^D$ where the knowledge conflicts with $\mathcal{E}$ are erased, the new knowledge boundary shrinks after the edit.
% \paragraph{Ignoring Static Knowledge} Existing work entirely neglects the static knowledge in the task formulation. They neither provide an explicit definition for these knowledge nor enable people to infer the static knowledge implicitly. We provide two empirical inference for the static knowledge set which are proved inapplicable.
% \begin{itemize} h leads to different conclusions. A typical example of this is shown in Figure~\ref{fig:dilemma}. 
% \end{itemize}

% \paragraph{Incomprehensive Evaluation} Existing methods mainly evaluate models on $\mathcal{E}$ and unchanged knowledge $\mathcal{R} \setminus \mathcal{S}$, which is unrelated to logical deduction. They fail to perform more comprehensive evaluations on $\mathcal{K}^\mathcal{E}$. 

% \subsection{Empirical Results}
% \label{sec:empirical}



==> Inserts/0dilemma.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{Inserts/figure0.drawio.pdf}
    \vspace{-15pt}
    \caption{Dilemma under current triple-based setting for knowledge editing. Since we did not point out the static knowledge set which should stay unchanged and base our reasoning on, it is hard to decide how to correctly make the edit. Candidate static knowledge set for this example: 1.\textit{\{Tokyo is in Japan.\}} 2.\textit{\{The Effiel Tower in in France.\}}}
    \label{fig:dilemma}
    % \vspace{-10pt}
\end{figure}
